Une approche combinatoire pour le r\'esultant multivari\'e. Le r\'esultant multivari\'e pour les enfants motiv\'es

We provide, in a 474 pages study, a comprehensive and self-contained treatment of Resultant Theory for a homogeneous system of polynomials with several variables (as many variables as of polynomials). In a non classical way, we use the multiplicative structure of finite free resolutions, by applying it to the complex homogeneous components of the Koszul complex of the system, and this in any degree. Moreover, these complexes have Macaulay decompositions. These three pillars, multiplicative structure, Koszul complex, Macaulay decomposition, allow to establish, surprisingly to us, remarkable binomial relations between 3 families of scalars resulting from the differentials of that complexes. These binomial relations generate several notable results, like a determinantal expression of a certain denominator, depending only on the first differential, and provide in particular formulas expressing the resultant. We have explored more deeply the case of the critical degree delta. This degree produces a fundamental linear form on the homogeneous polynomial component of degree delta, including the resultant. And this fundamental linear form has allowed us to highlight a certain number of remarkable properties. Key words: Elimination theory, homogeneous polynomial system, resultant, determinant of complexes, Cayley determinant, computational algebra, finitefree resolution, Koszul complex, Euler characteristic, Grade, Multiplicative structure, Macaulay decomposition, Fitting invariants, MacRae invariant, regular sequence.

==> 0-CodeBordermatrix.tex <==
\makeatletter
% Tentative du 03 Janvier 2022. Je commente dans le corps des macros tous les \newdimen
% que je déclare ici
\newdimen\@leftbwd%
\newdimen\@rightbwd%
\newdimen\@lastrowht%
\newdimen\@firstrowht%
\newdimen\@lastcolwd%
%
\def\NorthEastBordermatrix#1{%
\begingroup
  \m@th % mathsurround stuff
  % compute bracket width
  \setbox\z@\hbox{$\left [ \right.$}
  % \newdimen\@leftbwd
  \@leftbwd\wd\z@
  \setbox\z@\hbox{$\left.\right]$}
  % \newdimen\@rightbwd
  \@rightbwd\wd\z@
  % Define carriage-return for array rows
  \def\cr{\crcr\noalign{\global\let\cr\endline}} % for a safer \cr
  \def\\{\cr}
  % Set box0 to contain the matrix without bracket
  \setbox\z@\vbox{%
    \ialign{ 
      \hfil$##$\hfil && \quad \hfil$##$\hfil \crcr
      #1 \crcr 
    }}%
  % Determine the last row height
  % Extract last row from box 0 and measure its height
  \setbox\thr@@\vbox{\unvcopy\z@\global\setbox\tw@\lastbox}
  \setbox\tw@\vbox{\hrule\box\tw@\hrule}  
  % \newdimen\@lastrowht
  \@lastrowht\ht\tw@
  % Determine the first row height
  % by removing one row at a time from the content of box 0 (copied to box 3).   
  % If, after removing a row, the height of the box is less than 4pt, we rollback
  % one step and that is the first row's height
  \loop
    \ifdim\ht\thr@@>0pt
      \setbox\tw@\copy\thr@@
      \setbox\thr@@\vbox{%
        \unvbox\thr@@
        \loop% Remove kern, skip, and penalty until we found a box to remove
          \unkern\unskip\unpenalty
          \global\setbox\@ne\lastbox
          \ifvoid\@ne
        \repeat
      }
  \repeat
  \setbox\tw@\vbox{\hrule\copy\@ne\hrule} 
  % \newdimen\@firstrowht
  \@firstrowht\ht\tw@
  % Determine the last column width
  % After above, the first row is stored in box 1 and we extract the last
  % column and measure its width
  \setbox\tw@\hbox{%
    \unhcopy\@ne
    \loop
      \unkern\unskip\unpenalty
      \global\setbox\thr@@\lastbox
      \ifvoid\thr@@
    \repeat
  }
  % \newdimen\@lastcolwd
  \@lastcolwd\wd\thr@@
  % Put the bracket into the matrix:
  % First right shift for first column's width, and put the opening bracket, then
  % left shift to original position to put the matrix, and then shift left to close
  % the bracket and shift back to right.
  % The matrix, however, is also shifted to reflect the desired height of bracket,
  \setbox\tw@\hbox{$
    \left [
    \vcenter{%
     \kern-1.01\@firstrowht
      \unvcopy \z@
     \kern0.4\@lastrowht
          }
    \kern-\@lastcolwd
    \right ]
    \kern-\@rightbwd\kern\@lastcolwd
  $}
 % Print the result
 \setbox\tw@\vbox{\kern\@firstrowht\box\tw@}
 \box\tw@
 \endgroup
}
\makeatother  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\NorthEastBorderdet#1{%
\begingroup
  \m@th % mathsurround stuff
  % compute bracket width
  \setbox\z@\hbox{$\left | \right.$}
  % \newdimen\@leftbwd
  \@leftbwd\wd\z@
  \setbox\z@\hbox{$\left.\right|$}
  % \newdimen\@rightbwd
  \@rightbwd\wd\z@
  % Define carriage-return for array rows
  \def\cr{\crcr\noalign{\global\let\cr\endline}} % for a safer \cr
  \def\\{\cr}
  % Set box0 to contain the matrix without bracket
  \setbox\z@\vbox{%
    \ialign{ 
      \hfil$##$\hfil && \quad \hfil$##$\hfil \crcr
      #1 \crcr 
    }}%
  % Determine the last row height
  % Extract last row from box 0 and measure its height
  \setbox\thr@@\vbox{\unvcopy\z@\global\setbox\tw@\lastbox}
  \setbox\tw@\vbox{\hrule\box\tw@\hrule}  
  % \newdimen\@lastrowht
  \@lastrowht\ht\tw@
  % Determine the first row height
  % by removing one row at a time from the content of box 0 (copied to box 3).   
  % If, after removing a row, the height of the box is less than 4pt, we rollback
  % one step and that is the first row's height
  \loop
    \ifdim\ht\thr@@>0pt
      \setbox\tw@\copy\thr@@
      \setbox\thr@@\vbox{%
        \unvbox\thr@@
        \loop% Remove kern, skip, and penalty until we found a box to remove
          \unkern\unskip\unpenalty
          \global\setbox\@ne\lastbox
          \ifvoid\@ne
        \repeat
      }
  \repeat
  \setbox\tw@\vbox{\hrule\copy\@ne\hrule} 
  % \newdimen\@firstrowht
  \@firstrowht\ht\tw@
  % Determine the last column width
  % After above, the first row is stored in box 1 and we extract the last
  % column and measure its width
  \setbox\tw@\hbox{%
    \unhcopy\@ne
    \loop
      \unkern\unskip\unpenalty
      \global\setbox\thr@@\lastbox
      \ifvoid\thr@@
    \repeat
  }
  % \newdimen\@lastcolwd
  \@lastcolwd\wd\thr@@
  % Put the bracket into the matrix:
  % First right shift for first column's width, and put the opening bracket, then
  % left shift to original position to put the matrix, and then shift left to close
  % the bracket and shift back to right.
  % The matrix, however, is also shifted to reflect the desired height of bracket,
  \setbox\tw@\hbox{$
    \left |
    \vcenter{%
     \kern-1.01\@firstrowht
      \unvcopy \z@
     \kern0.4\@lastrowht
          }
    \kern-\@lastcolwd
    \right |
    \kern-\@rightbwd\kern\@lastcolwd
  $}
 % Print the result
 \setbox\tw@\vbox{\kern\@firstrowht\box\tw@}
 \box\tw@
 \endgroup
}
\makeatother  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\def\EastBordermatrix#1{%
\begingroup
  \m@th % mathsurround stuff
  % compute bracket width
  \setbox\z@\hbox{$\left [ \right.$}
  % \newdimen\@leftbwd
  \@leftbwd\wd\z@
  \setbox\z@\hbox{$\left.\right]$}
  % \newdimen\@rightbwd
  \@rightbwd\wd\z@
  % Define carriage-return for array rows
  \def\cr{\crcr\noalign{\global\let\cr\endline}} % for a safer \cr
  \def\\{\cr}
  % Set box0 to contain the matrix without bracket
  \setbox\z@\vbox{%
    \ialign{ 
      \hfil$##$\hfil && \quad \hfil$##$\hfil \crcr
      #1 \crcr 
    }}%
  % Determine the last row height
  % Extract last row from box 0 and measure its height
  \setbox\thr@@\vbox{\unvcopy\z@\global\setbox\tw@\lastbox}
  \setbox\tw@\vbox{\hrule\box\tw@\hrule}  
  % \newdimen\@lastrowht
  \@lastrowht\ht\tw@
  % Determine the first row height
  % by removing one row at a time from the content of box 0 (copied to box 3).   
  % If, after removing a row, the height of the box is less than 4pt, we rollback
  % one step and that is the first row's height
  \loop
    \ifdim\ht\thr@@>0pt
      \setbox\tw@\copy\thr@@
      \setbox\thr@@\vbox{%
        \unvbox\thr@@
        \loop% Remove kern, skip, and penalty until we found a box to remove
          \unkern\unskip\unpenalty
          \global\setbox\@ne\lastbox
          \ifvoid\@ne
        \repeat
      }
  \repeat
  \setbox\tw@\vbox{\hrule\copy\@ne\hrule} 
  % \newdimen\@firstrowht
  \@firstrowht\ht\tw@
  % Determine the last column width
  % After above, the first row is stored in box 1 and we extract the last
  % column and measure its width
  \setbox\tw@\hbox{%
    \unhcopy\@ne
    \loop
      \unkern\unskip\unpenalty
      \global\setbox\thr@@\lastbox
      \ifvoid\thr@@
    \repeat
  }
  % \newdimen\@lastcolwd
  \@lastcolwd\wd\thr@@
  % Put the bracket into the matrix:
  % First right shift for first column's width, and put the opening bracket, then
  % left shift to original position to put the matrix, and then shift left to close
  % the bracket and shift back to right.
  % The matrix, however, is also shifted to reflect the desired height of bracket,
  \setbox\tw@\hbox{$
    \left [
    \vcenter{%
      \unvcopy \z@
     \kern0.4\@lastrowht
          }
    \kern-\@lastcolwd
    \right ]
    \kern-\@rightbwd\kern\@lastcolwd
  $}
 % Print the result
 \setbox\tw@\vbox{\kern\@firstrowht\box\tw@}
 \box\tw@
 \endgroup
}
\makeatother  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\EastBorderdet#1{%
\begingroup
  \m@th % mathsurround stuff
  % compute bracket width
  \setbox\z@\hbox{$\left | \right.$}
  % \newdimen\@leftbwd
  \@leftbwd\wd\z@
  \setbox\z@\hbox{$\left.\right |$}
  % \newdimen\@rightbwd
  \@rightbwd\wd\z@
  % Define carriage-return for array rows
  \def\cr{\crcr\noalign{\global\let\cr\endline}} % for a safer \cr
  \def\\{\cr}
  % Set box0 to contain the matrix without bracket
  \setbox\z@\vbox{%
    \ialign{ 
      \hfil$##$\hfil && \quad \hfil$##$\hfil \crcr
      #1 \crcr 
    }}%
  % Determine the last row height
  % Extract last row from box 0 and measure its height
  \setbox\thr@@\vbox{\unvcopy\z@\global\setbox\tw@\lastbox}
  \setbox\tw@\vbox{\hrule\box\tw@\hrule}  
  % \newdimen\@lastrowht
  \@lastrowht\ht\tw@
  % Determine the first row height
  % by removing one row at a time from the content of box 0 (copied to box 3).   
  % If, after removing a row, the height of the box is less than 4pt, we rollback
  % one step and that is the first row's height
  \loop
    \ifdim\ht\thr@@>0pt
      \setbox\tw@\copy\thr@@
      \setbox\thr@@\vbox{%
        \unvbox\thr@@
        \loop% Remove kern, skip, and penalty until we found a box to remove
          \unkern\unskip\unpenalty
          \global\setbox\@ne\lastbox
          \ifvoid\@ne
        \repeat
      }
  \repeat
  \setbox\tw@\vbox{\hrule\copy\@ne\hrule} 
  % \newdimen\@firstrowht
  \@firstrowht\ht\tw@
  % Determine the last column width
  % After above, the first row is stored in box 1 and we extract the last
  % column and measure its width
  \setbox\tw@\hbox{%
    \unhcopy\@ne
    \loop
      \unkern\unskip\unpenalty
      \global\setbox\thr@@\lastbox
      \ifvoid\thr@@
    \repeat
  }
  % \newdimen\@lastcolwd
  \@lastcolwd\wd\thr@@
  % Put the bracket into the matrix:
  % First right shift for first column's width, and put the opening bracket, then
  % left shift to original position to put the matrix, and then shift left to close
  % the bracket and shift back to right.
  % The matrix, however, is also shifted to reflect the desired height of bracket,
  \setbox\tw@\hbox{$
    \left |
    \vcenter{%
      \unvcopy \z@
     \kern0.4\@lastrowht
          }
    \kern-\@lastcolwd
    \right |
    \kern-\@rightbwd\kern\@lastcolwd
  $}
 % Print the result
 \setbox\tw@\vbox{\kern\@firstrowht\box\tw@}
 \box\tw@
 \endgroup
}
\makeatother  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

